Fault-Tolerant Control of Degrading Systems with On-Policy Reinforcement Learning

We propose a novel adaptive reinforcement learning control approach for fault tolerant control of degrading systems that is not preceded by a fault detection and diagnosis step. Therefore, \textit{a priori} knowledge of faults that may occur in the system is not required. The adaptive scheme combines online and offline learning of the on-policy control method to improve exploration and sample efficiency, while guaranteeing stable learning. The offline learning phase is performed using a data-driven model of the system, which is frequently updated to track the system's operating conditions. We conduct experiments on an aircraft fuel transfer system to demonstrate the effectiveness of our approach.

==> 2-litreview.tex <==
\section{Background}

% Literature review on:
%  - FTC
%  - Model-based FTC
%  - FTC with degrading faults
%  - Reinforcement learning for FTC

% Define FTC
The architecture of FTC systems is surveyed in \cite{bla97}. FTC detects faulty conditions, accommodates faults during system operation, and slows down the progress to complete system failures. This is differentiated from fail-safe systems, where redundancies prevent failure conditions from occurring in the first place. Thus FTC approaches require comparatively fewer hardware add-ons to the system as the focus is on mitigating faults after the fact by adapting the controller to the changing conditions in the system.

% Survey of FTC - OPTIONAL: this was lifted word-for-word from the previous paper and needs to be reworded anyways. If you are out of space then omit this paragraph.
\cite{pat97} surveys constituent research areas of FTC. Fault-tolerant supervision has been explored in several fields including probabilistic reasoning, fuzzy logic, and genetic algorithms. With recent advances in computing and communication systems, the fault-tolerant control problem is being applied to a wide range of industrial and transportation applications, primarily due to increased safety and reliability demands beyond what a conventional control system can offer \cite{yen2003online, zhang2008}. These applications include aerospace, nuclear power, automotive, manufacturing and other process industries, and fault tolerance is no longer limited to high-end systems. Consumer products, such as automobiles, increasingly dependent on microelectronic and mechatronic systems, on-board communication networks and software, are pushing the frontiers of fault tolerance.

% model-based FTC with degrading faults
There is ample literature on model-based FTC with degrading faults. \cite{noura2000fault} discusses FTC under two regimes: sensor faults and actuator faults. In the former, the controller does not need to respond as the fault only lies with perception of state. Whereas in the later, a change in control law is required. In both cases accurate fault detection and diagnosis is required.

In (\cite{zhang2003fault, jiang2006accepting}), performance degraded reference models are used to achieve fault tolerant control. Once a fault is diagnosed, a reference model matching the fault signature is employed for control. This can be applied to progressively degrading systems by generating reference models for various levels of degradation. This, however, requires \textit{a priori} knowledge of possible faults and an ability to generate accurate system models.

% RL based FTC control
RL-based control is an active area of research. It has been applied to robotics (\cite{kober2013reinforcement}), board games (\cite{silver2018general}), and smart buildings (\cite{naug2019online}) among other things. \cite{lewis2012reinforcement} discusses application of RL to designing optimal and adaptive controllers. Adaptive controllers develop and learn from a system model on the fly, but at the cost of true optimality in control. \cite{liu2016} uses neural networks to approximate tracking error. The focus is on making the training of the networks faster so the system model can be updated regularly in response to faults to generate a control policy. Both incipient and abrupt faults are demonstrated on a non-linear system. \cite{zhao2017} develops an RL-based fault-tolerant controller for actuator faults. Instead of rewards and values, costs an objective functions are used. The objective function is a cumulative sum of the actuator fault and the cost of the control action over time. The goal is to minimize the objective function over actions.

In our previous work, \cite{ahmed2018comparison}, a RL-based fault-tolerant controller was proposed for abrupt faults. Faults were simulated on a fuel tank system of a C-130 aircraft. A value iteration algorithm was used with a polynomial action value function from which policy was derived. The controller showed robustness to Gaussian sensor noise in comparison to model predictive control. However, the proposed algorithm learned a policy offline, and with knowledge of diagnosed faults, on a system model. The learned policy was then transferred to the actual system for FTC. In this work, we iterate on our previous endeavour and present an online RL control algorithm for degrading systems that does not need the fault diagnosis step.

